Estimation of Microphone Clusters in Acoustic Sensor Networks using Unsupervised Federated Learning

In this paper we present a privacy-aware method for estimating source-dominated microphone clusters in the context of acoustic sensor networks (ASNs). The approach is based on clustered federated learning which we adapt to unsupervised scenarios by employing a light-weight autoencoder model. The model is further optimized for training on very scarce data. In order to best harness the benefits of clustered microphone nodes in ASN applications, a method for the computation of cluster membership values is introduced. We validate the performance of the proposed approach using clustering-based measures and a network-wide classification task.

==> figures/federated.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Flowchart: Magnetic Disk [id:dp049474331058075416] 
\draw   (309.3,38.25) -- (309.3,83.75) .. controls (309.3,90.52) and (288.19,96) .. (262.15,96) .. controls (236.11,96) and (215,90.52) .. (215,83.75) -- (215,38.25)(309.3,38.25) .. controls (309.3,45.02) and (288.19,50.5) .. (262.15,50.5) .. controls (236.11,50.5) and (215,45.02) .. (215,38.25) .. controls (215,31.48) and (236.11,26) .. (262.15,26) .. controls (288.19,26) and (309.3,31.48) .. (309.3,38.25) -- cycle ;
%Flowchart: Alternative Process [id:dp20957244779600814] 
\draw   (159,159.18) .. controls (159,155.77) and (161.77,153) .. (165.18,153) -- (211.65,153) .. controls (215.06,153) and (217.83,155.77) .. (217.83,159.18) -- (217.83,182.15) .. controls (217.83,185.56) and (215.06,188.33) .. (211.65,188.33) -- (165.18,188.33) .. controls (161.77,188.33) and (159,185.56) .. (159,182.15) -- cycle ;
%Straight Lines [id:da5936191896828573] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (215,50.63) -- (170.5,50.18) -- (170.5,150) ;
\draw [shift={(170.5,153)}, rotate = 270] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da386928290761815] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (190.5,152.57) -- (190.5,70.04) -- (211.5,70.04) ;
\draw [shift={(214.5,70.04)}, rotate = 180] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Square [id:dp6468774428878161] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (159.5,61.54) -- (180.96,61.54) -- (180.96,83) -- (159.5,83) -- cycle ;

%Shape: Square [id:dp021283356429652844] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (176.69,101.73) -- (205.5,101.73) -- (205.5,130.55) -- (176.69,130.55) -- cycle ;
%Straight Lines [id:da043222509694045286] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (245.5,94.57) -- (245.5,113.57) -- (245.5,150) ;
\draw [shift={(245.5,153)}, rotate = 270] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da6171304175035741] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (278.89,153) -- (278.89,122.57) -- (278.89,98.57) ;
\draw [shift={(278.89,95.57)}, rotate = 450] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Square [id:dp5965756244650497] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (234.5,101.54) -- (255.96,101.54) -- (255.96,123) -- (234.5,123) -- cycle ;
%Shape: Square [id:dp7911788257837484] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (264.69,115.73) -- (293.5,115.73) -- (293.5,144.55) -- (264.69,144.55) -- cycle ;
%Straight Lines [id:da45845896346006954] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (309.5,48.63) -- (359.5,48.63) -- (359.5,149) ;
\draw [shift={(359.5,152)}, rotate = 270] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Square [id:dp30268681083034266] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (349.5,61.54) -- (370.96,61.54) -- (370.96,83) -- (349.5,83) -- cycle ;
%Straight Lines [id:da8964423971998534] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (333.5,151.63) -- (333.5,70.63) -- (312.5,70.63) ;
\draw [shift={(309.5,70.63)}, rotate = 360] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da4333853876385376] 
\draw    (159.5,170.63) -- (218.83,170.33) ;
%Flowchart: Alternative Process [id:dp8288106091536687] 
\draw   (236,159.18) .. controls (236,155.77) and (238.77,153) .. (242.18,153) -- (288.65,153) .. controls (292.06,153) and (294.83,155.77) .. (294.83,159.18) -- (294.83,182.15) .. controls (294.83,185.56) and (292.06,188.33) .. (288.65,188.33) -- (242.18,188.33) .. controls (238.77,188.33) and (236,185.56) .. (236,182.15) -- cycle ;
%Flowchart: Alternative Process [id:dp22370502556066585] 
\draw   (314,159.18) .. controls (314,155.77) and (316.77,153) .. (320.18,153) -- (366.65,153) .. controls (370.06,153) and (372.83,155.77) .. (372.83,159.18) -- (372.83,182.15) .. controls (372.83,185.56) and (370.06,188.33) .. (366.65,188.33) -- (320.18,188.33) .. controls (316.77,188.33) and (314,185.56) .. (314,182.15) -- cycle ;
%Straight Lines [id:da8802911353380236] 
\draw    (235.5,170.63) -- (294.83,170.33) ;
%Straight Lines [id:da2854194567550412] 
\draw    (313.5,170.63) -- (372.83,170.33) ;
%Shape: Rectangle [id:dp5972387342060843] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (319.5,102.73) -- (351.5,102.73) -- (351.5,131.5) -- (319.5,131.5) -- cycle ;

% Text Node
\draw (243,60) node [anchor=north west][inner sep=0.75pt]   [align=left] {Server};
% Text Node
\draw (162,157.02) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{37.304392pt}\setlength\topsep{0pt}
\begin{center}
Client 1
\end{center}

\end{minipage}};
% Text Node
\draw (239.5,105.54) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathbf{\theta }$};
% Text Node
\draw (354.5,64.54) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathbf{\theta }$};
% Text Node
\draw (172,171.63) node [anchor=north west][inner sep=0.75pt]   [align=left] {SGD};
% Text Node
\draw (318.69,109.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathbf{\Delta \theta_{M} }$};
% Text Node
\draw (264.69,121.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathbf{\Delta \theta_{2} }$};
% Text Node
\draw (176.69,107.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathbf{\Delta \theta_{1} }$};
% Text Node
\draw (163.5,64.54) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathbf{\theta }$};
% Text Node
\draw (239,157.02) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{37.304392pt}\setlength\topsep{0pt}
\begin{center}
Client 2
\end{center}

\end{minipage}};
% Text Node
\draw (249,171.63) node [anchor=north west][inner sep=0.75pt]   [align=left] {SGD};
% Text Node
\draw (315,157.02) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.130608pt}\setlength\topsep{0pt}
\begin{center}
Client M
\end{center}

\end{minipage}};
% Text Node
\draw (327,171.63) node [anchor=north west][inner sep=0.75pt]   [align=left] {SGD};
% Text Node
\draw (297,168.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};


\end{tikzpicture}
